Efficient Online Classification and Tracking on Resource-constrained IoT Devices

Timely processing has been increasingly required on smart IoT devices, which leads to directly implementing information processing tasks on an IoT device for bandwidth savings and privacy assurance. Particularly, monitoring and tracking the observed signals in continuous form are common tasks for a variety of near real-time processing IoT devices, such as in smart homes, body-area and environmental sensing applications. However, these systems are likely low-cost resource-constrained embedded systems, equipped with compact memory space, whereby the ability to store the full information state of continuous signals is limited. Hence, in this paper, we develop solutions of efficient timely processing embedded systems for online classification and tracking of continuous signals with compact memory space. Particularly, we focus on the application of smart plugs that are capable of timely classification of appliance types and tracking of appliance behavior in a standalone manner. We implemented a smart plug prototype using low-cost Arduino platform with small amount of memory space to demonstrate the following timely processing operations: (1) learning and classifying the patterns associated with the continuous power consumption signals, and (2) tracking the occurrences of signal patterns using small local memory space. Furthermore, our system designs are also sufficiently generic for timely monitoring and tracking applications in other resource-constrained IoT devices.

==> sketch.tex <==
\section{Multiplexed Sketches} \label{sec:sketch}

\subsection{Preliminaries}

If we can record all flow IDs that appear in each time slot, that is we have $f_{i}(t)$ for every $i$ and $t$, then it is straightforward to compute the flow correlations. However, there are two reasons that may render such a method impractical. First, the huge space complexity will be a great burden for distributed tracking, since the recorded information must be transmitted. Second and more important, the recording speed is often much slower than the link speed (e.g. $\ge 10$ Gbps) , and packet sampling or flow sampling has to be used~\cite{netflow,superspreader,cSamp-T}, which will greatly affect the accuracy. These two shortcomings will be further explained in the evaluation section.

So in this paper we concern online tracking by developing space-efficient randomized data structures and corresponding high speed streaming algorithms. Streaming algorithms can read input data in only one pass, and provide approximate answers to some specific problems with sub-linear space relative to the input size~\cite{streaming}. This section explains the data structures on a single tracker, while the distributed deployment will be discussed in section \ref{sec:system}.

We first define some notations. Consider a sequence of items $X \triangleq (e_{1},e_{2},...)$, where each item $e_{i}$ belongs to one of the types ${\sf N} \triangleq \{{\sf 1}, {\sf 2},..., {\sf n}\}$. Denote the frequency of type ${\sf i}$ in $X$ as ${\rm Freq}({\sf i})$, and the number of distinct items in $X$ as $|X|$. For example, $X=({\sf 1}, {\sf 2}, {\sf 1}, {\sf 3}, {\sf 3}, {\sf 1})$ and ${\sf N} = \{{\sf 1}, {\sf 2},..., {\sf 4}\}$, then ${\rm Freq}({\sf 1})=3$, ${\rm Freq}({\sf 4})=0$, and $|X| = 3$. Given two sequences $X$ and $Y$, we define their join size as $X \Join Y \triangleq \sum_{{\sf i} \in {\sf N}} {\rm Freq}_X(\sf i) \cdot {\rm Freq}_Y(\sf i)$, where ${\rm Freq}_X(\sf i)$ and ${\rm Freq}_Y(\sf i)$ are the frequencies of type ${\sf i}$ in sequences $X$ and $Y$ respectively.

For our problem, each flow $i \in {\cal F}$ can be regarded as a sequence of activated time slots:
\begin{equation}
F_{i} \triangleq \big(t : f_{i}(t) = 1, t \in {\cal T} \big) 
\end{equation}
where ${\cal T}$ is a bounded epoch of time. For example, $ F_{i} = (1, 2, 6)$ means that flow $i$ occurs in time slots $1, 2$, and $6$. In fact, $F_{i}$ is a degenerated sequence, in the sense that each type $t \in {\cal T}$ occurs at most once. Then it is easy to verify that, ${\sf Cor}(i,j)$ can be rewritten as either $|F_{i} \cap F_{j}|$ or $F_{i} \Join F_{j}$. 

Given $F_{i}$ and $F_{j}$ as input, there exist many streaming algorithms for estimating $|F_{i} \cap F_{j}|$ (e.g., ~\cite{PU,linear}) or $F_{i} \Join F_{j}$ (e.g., ~\cite{AGMS,Fast-AGMS}). However, all these algorithms implement a common paradigm: they maintain a compact {\em sketch} data structure for each sequence. However, for our flow correlation tracking problem, it is not uncommon that millions of (or even more) flows or groups should be handled simultaneously in a large network, and it is not feasible to maintain a separate {\em sketch} for each of them since the space complexity will be linear to the total number of flows and groups.

\subsection{Design of Multiplexed Sketches} \label{sec:Multiplexed}

Now we describe our {\em multiplexed sketches} which significantly reduce the space complexity. The basic idea is that we only maintain a fixed number of sketches, and randomly assign a flow (or group) to one (or some) of the sketches by hash function. Then each sketch is updated only by those flows that are assigned to the particular sketch. Although the idea is simple, it is not clear how to balance the space complexity and the accuracy of estimation, because multiple random behavior is involved. Hence, we also provide an in-depth analysis of the trade-off between space and accuracy in multiplexed sketches.


\subsubsection{Multiplexed Proportional Union (MPU) Sketches}

We use an array of ${\sf p} \times {\sf m} \times {\sf s}$ counters, denoted as ${\mathbf C}_{k}[r][\ell]$ where $1 \le k \le {\sf p}, 1 \le r \le {\sf m}, 1 \le \ell \le {\sf s}$, and ${\sf p} + 2$ hash functions randomly chosen from some pair-wise independent hash families:\footnote{A family of hash functions $H$ from $\{1,...,N\}$ to $\{1,...,M\}$ is called pair-wise independent, if ${\mathbb P}_{h \in H}\{h({\sf i})={\sf a}, h({\sf j})={\sf b}\} = 1/M^{2}$ for every ${\sf i}, {\sf j} \in \{1,...,N\}$ such that ${\sf i} \ne {\sf j}$, and every ${\sf a}, {\sf b} \in  \{1,...,M\}$. Four-wise independent is defined in a similar manner. There are efficient implementations of these hash functions \cite{universal}.}
\[
h_{k} : {\cal F} \mapsto \{1,...,{\sf m}\}, \ \ 
g : {\cal T} \mapsto\{1,...,{\sf s}\}, \ \ 
\phi : {\cal T} \mapsto \{1,...,{\sf w}\} 
\]
Initially, the value of each counter is set to be ${\sf w} + 1$. In each time slot $t$, if flow $i$ occurs, we use Algorithm \ref{alg:UpdateMPU} to update the counters. The idea is that we treat each column of counters as a compact sketch, and assign a flow $i$ to ${\sf p}$ sketches ${\mathbf C}_{k}[h_{k}(i)]$ ($1 \le k \le {\sf p}$), one in each block. Then we update a counter indexed by $g(t)$ in each of the ${\sf p}$ sketches, as indicated by the black squares in Fig. \ref{fig:MPU}. 

\begin{figure}[t]
\centering
%\epsfig{file=fig-MPU.eps, width=0.5\textwidth}
\caption{An illustraion of Multiplex PU sketches.}
\label{fig:MPU}
\end{figure}


\begin{algorithm}[h] 
\caption{UpdateMPU(flow $i$, time slot $t$)}
\label{alg:UpdateMPU}
\begin{algorithmic}[1]
  \If{$f_i(t) == 1$}
  \For{$k = 1, ..., {\sf p}$}
    \State ${\bf C}_{k}[h_{k}(i)][g(t)] \leftarrow \min\big\{{\bf C}_{k}[h_{k}(i)][g(t)], \phi(t)\big\}$;
  \EndFor
  \EndIf
\end{algorithmic}
\end{algorithm} 


\begin{algorithm}[h] 
\caption{EstimateMPU(flow $i$, flow $j$)}
\label{alg:EstimateMPU}
\begin{algorithmic}[1]
  \State $a \leftarrow 0; b \leftarrow 0; c \leftarrow 0$;
  \For{$\ell = 1, ...,{\sf s}$}
    \State $min \leftarrow \displaystyle\min_{1 \le k \le {\sf p}}\{{\bf C}_{k}[h_{k}(i)][\ell], {\bf C}_{k}[h_{k}(j)][\ell]\}$;
    \If{$min == \displaystyle\max_{1 \le k \le {\sf p}}\{{\bf C}_{k}[h_{k}(i)][\ell], {\bf C}_{k}[h_{k}(j)][\ell]\}$}
      \State $a \leftarrow a+1$;
    \EndIf
    \If{$min \le {\sf w}$}
      \State $b \leftarrow b+1$;
    \EndIf
    \State $c \leftarrow c+min$;
  \EndFor
  \State return $a \cdot b / c$;
\end{algorithmic}  
\end{algorithm} 


To estimate ${\sf Cor}(i,j)$, we use Algorithm \ref{alg:EstimateMPU}. The basic idea is that, if ${\sf m}$ is large, then with high probability no flow other than $i$ can be assigned to the same ${\sf p}$ sketches as $i$. Hence, we can estimate $|F_{i} \cap F_{j}|$ by the corresponding $2{\sf p}$ sketches that $i$ and $j$ are assigned to. In our algorithms, each column of counters works similar to a Proportional Union sketch~\cite{PU} proposed for cardinality estimation. The differences are: (1) PU sketch focuses more on extremely small space, so it uses continuous counters and log function, while MPU trades off some space for higher speed by discretizing the counters and using much simpler arithmetic functions; (2) The estimation algorithm of MPU must consider multiple flows sharing the same column. To give more precise results on the trade-off between space and accuracy, we provide some analytical results as follows.

\begin{lemma}
\label{lemma:MPU-flowcollision}
The probability that there exist two flows being assigned to the same ${\sf p}$ rows is less than $|{\cal F}|^{2}/(2{\sf m}^{{\sf p}})$.
\end{lemma}
\begin{lemma}
\label{lemma:MPU-variance}
If no two flows are assigned to the same ${\sf p}$ rows, and assume the hash function $\phi$ is a perfect continuous uniform hash $\phi : {\cal T} \to [0,1]$, then for any pair of flows $i$ and $j$, Algorithm \ref{alg:EstimateMPU} returns ${\sf \widetilde{Co}r}(i,j)$ as an asymptotically unbiased estimation of ${\sf Cor}(i,j)$, and ${\rm Var}({\sf \widetilde{Co}r}(i,j)) \le {\sf Cor}(i,j) \cdot |{\cal T}|/{\sf s}$.
\end{lemma}
\begin{lemma}
\label{lemma:MPU-countercollision}
The probability that using a discrete hash function $\phi : {\cal T} \to \{1,...,{\sf w}\}$ (instead of a continuous hash) will decrease the accuracy of estimation is less than $|{\cal T}|^{2}/(2{\sf w}{\sf s})$.
\end{lemma}

Combining these results, MPU can provide an ($\epsilon,\delta$)-accurate estimation.

\begin{theorem}
\label{theorem:MPU-bound}
Let ${\sf \widetilde{Co}r}(i,j)$ be the median estimation of $O(\log(1/\delta))$ independent copies of MPU sketches, where ${\sf s}=O(1/\epsilon^{2})$, ${\sf w}=O(\epsilon^{2} \cdot |{\cal T}|^{2})$, ${\sf m}=O((2|{\cal F}|)^{2/{\sf p}})$, and ${\sf p}$ can be an arbitrary integer. Then,
 ${\mathbb P}(|{\sf \widetilde{Co}r}(i,j)-{\sf Cor}(i,j)| \ge \epsilon \cdot \sqrt{{\sf Cor}(i,j) \cdot |{\cal T}|}) \le \delta$, and the total space used is 
\[
O(\log(1/\delta) \cdot 1/\epsilon^{2} \cdot \log(\epsilon \cdot |{\cal T}|) \cdot {\sf p} \cdot (2|{\cal F}|)^{2/{\sf p}}) \mbox{\ bits} 
\]

In the extreme case, we can let ${\sf p}=\log(|{\cal F}|)$, then the space complexity is $O(\log(1/\delta) \cdot 1/\epsilon^{2} \cdot \log(\epsilon \cdot |{\cal T}|) \cdot \log(|{\cal F}|))$, which only increase logarithmically with respect to $|{\cal F}|$.
\end{theorem}

\begin{corollary}
\label{corollary:MPU-bound}
${\mathbb P}(|{\sf \widetilde{Co}r}(i,j)-{\sf Cor}(i,j)| \ge \epsilon \cdot |{\cal T}|) \le \delta$, because ${\sf Cor}(i,j) \le |{\cal T}|$.
\end{corollary}

It is worth to mention that the definition of ${\sf Cor}(i,j)$ requires $f_{i}(t)$ to be either zero or one, but in a real network, a flow may occur multiple times in a time slot. Nevertheless, {\em MPU} cares only the distinct items, and still works when updated on each packet arrival. 
Note that it requires $O({\sf p})$ update operations. In practice ${\sf p}$ should be a small integer such as 3 $\sim$ 5. However, for a hardware implementation with parallelization, ${\sf p}$ can be made larger to use less memory.


\subsection{Group-level Correlations}
\label{sec:group}

To track ${\sf GCor}(A,B)$, we can regard a group of flows as a sequence of items, which is the union of all items in the corresponding flows. If $f_{A}(t)$ is defined as an indicator of any flow in $A$ as in (${\sf g.1}$) Eqn.~(\ref{eqn:group-any}), then MPU can be used. If $f_{A}(t)$ is defined as the summation of flow occurrences as in (${\sf g.2}$) Eqn.~(\ref{eqn:group-sum}), then MTW can be used. In both cases, the only change to the corresponding algorithms is to take group ID instead of flow ID as input. All the above lemmas and theorems still hold.\footnote{In the statements, when necessary, the flow set ${\cal F}$ should be replaced by the group set ${\cal G}$, the flow correlation ${\sf Cor}(i,j)$ should be replaced by the group correlation ${\sf GCor}(A,B)$, and similarly for ${\sf Cor}_{k}$ and ${\sf RCor}_{k}$. Note that Corollary \ref{corollary:MPU-bound} still holds, but Corollary \ref{corollary:MTW-bound} may not, since the self group correlation ${\sf GCor}(A,A)$ is no longer bounded by $|{\cal T}|$ when Eqn.~(\ref{eqn:group-sum}) is used. } 

The aforementioned ``back-end service dependency'' can be tracked by estimating ${\sf GCor}(A,B)$ of the correpsonding groups $A$ and $B$. Now we provide two examples of some advanced tracking of group-level correlations:

{\bf Example 1}:
To track ``related service dependency'', we consider a sequence of tuples (srcIP, time slot), instead of a sequence of time slots. This is because we are interested in the same client accessing the two services in the same time slot. Simple modifications (that consider the tuple as a type) to the multiplexed sketches are sufficient to track such dependency. %\footnote{The hash functions $g$ and $\phi$ should be changed appropriately.}

{\bf Example 2}:
Sometimes, we may want to incorporate the relative order of activities, packet delay or time differences. For example, consider ${\sf Cor}^{\tau}(i,j)\!\triangleq\! \sum_{0 \le \omega \le \tau}\sum_{t \in {\cal T}}f_{i}(t) \cdot f_{j}(t+\omega)$, where $\tau$ is a small constant. That is, even when the activity in flow $j$ occurs a few time slots later than the activity of flow $i$, we still consider the two activities are correlated. By transformation, ${\sf Cor}^{\tau}(i,j)\!=\!\sum_{t \in {\cal T}}f_{i}(t)\sum_{0 \le \omega \le \tau} \cdot f_{j}(t+\omega)$, and we can construct a virtual group $G$, whose activity is $G(t)=\sum_{0 \le \omega \le \tau}f_{j}(t+\omega)$. Namely, all activities of flow $j$ in $[t, t+\tau]$ contribute to activities of $G$ in time slot $t$. So when we see flow $j$ in time slot $t$, we then call the appropriate Update($G$, $t-\omega$) for $0 \le \omega \le \tau$. Then, the correlation ${\sf Cor}^{\tau}(i,j)$ can be estimated, just as ${\sf Cor}(i,G)$. 

These examples demonstrate that, by appropriately changing the definitions of flow (sequence) and time slot (item type) of our algorithms to fit the need of specific problems, we can provide more powerful tracking capabilities.

